Large Model Based Referring Camouflaged Object Detection

Referring camouflaged object detection (Ref-COD) is a recently-proposed problem aiming to segment out specified camouflaged objects matched with a textual or visual reference. This task involves two major challenges: the COD domain-specific perception and multimodal reference-image alignment. Our motivation is to make full use of the semantic intelligence and intrinsic knowledge of recent Multimodal Large Language Models (MLLMs) to decompose this complex task in a human-like way. As language is highly condensed and inductive, linguistic expression is the main media of human knowledge learning, and the transmission of knowledge information follows a multi-level progression from simplicity to complexity. In this paper, we propose a large-model-based Multi-Level Knowledge-Guided multimodal method for Ref-COD termed MLKG, where multi-level knowledge descriptions from MLLM are organized to guide the large vision model of segmentation to perceive the camouflage-targets and camouflage-scene progressively and meanwhile deeply align the textual references with camouflaged photos. To our knowledge, our contributions mainly include: (1) This is the first time that the MLLM knowledge is studied for Ref-COD and COD. (2) We, for the first time, propose decomposing Ref-COD into two main perspectives of perceiving the target and scene by integrating MLLM knowledge, and contribute a multi-level knowledge-guided method. (3) Our method achieves the state-of-the-art on the Ref-COD benchmark outperforming numerous strong competitors. Moreover, thanks to the injected rich knowledge, it demonstrates zero-shot generalization ability on uni-modal COD datasets. We will release our code soon.

==> tables/prompts2.tex <==

\begin{table*}[!t]
\caption{Our prompts for multimodal LLM.}
  \centering
  \resizebox{\textwidth}{!}
   {
  % \begin{tabular}{l*{2}{c}}
  \begin{tabular}{c p{11cm}}
    \toprule
     Number & Content  \\
    \midrule
    Prompt \#1& `This is a picture of a [CLS] hidden in the background, please give me a brief description based only on the morphological information of a general [CLS] (Only describe physical characteristics, do not need to describe life habits and so on).No more than 50 words.' \\
    Prompt \#2& `Please use detailed language to describe the entire scene in the given image of a [CLS].No more than 30 words.' \\        
    Prompt \#3&  `Within this scene, how does the [CLS] blend in the environment? Please describe it from the perspective of [color] in one sentence.' \\
    Prompt \#4& `Within this scene, how does the [CLS] blend in the environment? Please describe it from the perspective of [texture] in one sentence.' \\
    Prompt \#5&  `Within this scene, how does the [CLS] blend in the environment? Please describe it from the perspective of [shape] in one sentence.' \\
    Prompt \#6& `Within this scene, how does the [CLS] blend in the environment? Please describe it from the perspective of [environment lightning condition] in one sentence.' \\
    \bottomrule
  \end{tabular}
 }
  
  \label{table:prompts}
\end{table*}



==> tables/table5.tex <==

\begin{table}[!t]
\caption{Ablation experiments on target and camouflaged scene knowledge. Baseline: Fine-tuning SAM~\cite{kirillov2023segment} using LoRA~\cite{hu2021lora}. $\uparrow/\downarrow$ denotes that the higher/lower the score, the better.}
  \centering
  \resizebox{0.45\textwidth}{!}
   {
  \begin{tabular}{l*{4}{c}}
    \toprule
    Setting &$\textit{S}_{m}\uparrow$ & $\alpha E\uparrow$ & $\textit{F}^{w}_{\beta}\uparrow$ & $\textit{M}\downarrow$  \\
    \midrule
    Baseline   &0.895 &0.888 &0.788 &0.023 \\
    Baseline+target knowledge  &0.906 &0.91 &0.817 &0.021\\
    Baseline+scene knowledge &0.903 &0.916 &0.820 &0.020 \\
    Baseline+both knowledge &0.910 &0.916 &0.828 &0.020 \\
    
    \bottomrule
  \end{tabular}
 }
  
  \label{table5}
\end{table}


